SYN-MAD 2022: Competition on Face Morphing Attack Detection Based on Privacy-aware Synthetic Training Data

This paper presents a summary of the Competition on Face Morphing Attack Detection Based on Privacy-aware Synthetic Training Data (SYN-MAD) held at the 2022 International Joint Conference on Biometrics (IJCB 2022). The competition attracted a total of 12 participating teams, both from academia and industry and present in 11 different countries. In the end, seven valid submissions were submitted by the participating teams and evaluated by the organizers. The competition was held to present and attract solutions that deal with detecting face morphing attacks while protecting people's privacy for ethical and legal reasons. To ensure this, the training data was limited to synthetic data provided by the organizers. The submitted solutions presented innovations that led to outperforming the considered baseline in many experimental settings. The evaluation benchmark is now available at: https://github.com/marcohuber/SYN-MAD-2022.

==> name.tex <==
\begin{table*}[]
\centering
\small
\begin{tabular}{llll} \hline
Solution              & Team Members                      & Affiliations                                 & Type \\ \hline \hline
Xception & Borut Batagelj, Andrej Kronov\v{s}ek, & Faculty of Computer and Information Science, & Academic            \\
              & Peter Peer                        & University of Ljubljana                      &                     \\ \hline
MorphHRNet            & Marija Ivanovska, Borut Batagelj, & Faculty of Electrical Engineering,           & Academic            \\
                      & Peter Peer, Vitomir \v{S}truc         & Faculty of Computer and Information Science, &                     \\
                      &                                   & University of Ljubljana                      &                     \\ \hline
E-CBAM@VCMI           & Pedro C. Neto, Tiago Gon\c{c}alves,   & INESC TEC, Faculty of Engineering,           & Academic            \\
                      & Ana F. Sequeira, Jaime S. Cardoso & University of Porto                          &                     \\ \hline
Con-Text Net (A/B)         & Jo\~{a}o Tremo\c{c}o, Miguel Louren\c{c}o     & Yoonik                                       & Industry            \\ \hline
VaMoS                 & Sergio Serra, Eduardo Cerme\~{n}o     & Vaelsys R\&D                                 & Industry            \\ \hline
Anonymous             & Anonymous                         & Anonymous                                    & mixed     \\  \hline
\end{tabular}
\vspace{0.5mm}
\caption{A summary of the valid submitted solutions, participating team members, affiliations, and type of institution. More details on the submitted algorithms are provided in Section  \ref{solutions}.}
\label{teams}
\end{table*}

\begin{table*}[]
\small
\centering
\resizebox{0.90\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Solution}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Input size}\\ \textbf{(in pixels)}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Architecture/}\\ \textbf{Model}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Loss function}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Evaluation data}\\ \textbf{during training}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Bounding box/}\\ \textbf{Landmarks?}\end{tabular}} \\ \hline
MorphHRNet & $256 \times 256$ & HRNet & \begin{tabular}[c]{@{}l@{}}Binary cross \\ entropy\end{tabular} & \begin{tabular}[c]{@{}l@{}}20\% of provided data, \\ FRLL, FERET \\ and FRGC morphs\end{tabular} & bounding box \\ \hline
Con-Text Net A & \begin{tabular}[c]{@{}l@{}}$128 \times 128$ \\ and $256 \times 256$\end{tabular} & 2xResNet-50 & \begin{tabular}[c]{@{}l@{}}Weighted Focal \end{tabular} & \begin{tabular}[c]{@{}l@{}}New Face Morphing Dataset\end{tabular} & landmarks \\ \hline
Xception & $299 \times 299$ & Xception net & \begin{tabular}[c]{@{}l@{}}Cross-entropy \end{tabular} & \begin{tabular}[c]{@{}l@{}}FRLL, FERET and \\ FRGC morphs\end{tabular} & \begin{tabular}[c]{@{}l@{}}other\\ alignment\end{tabular} \\ \hline
Con-Text Net B & \begin{tabular}[c]{@{}l@{}}$128 \times 128$\\ and $256 \times 256$\end{tabular} & 2xResNet-50 & \begin{tabular}[c]{@{}l@{}}Weighted Focal \end{tabular} & New Face Morphing Dataset & landmarks \\ \hline
E-CBAM@VCMI & $256 \times 256$ & \begin{tabular}[c]{@{}l@{}}4xResNet-50\\ with CBAM\end{tabular} & Cross-entropy  & \begin{tabular}[c]{@{}l@{}}25\% of the data for \\ different models\end{tabular} & no alignment \\ \hline
Anonymous & $256 \times 256$ & Hand-crafted+SVM & \begin{tabular}[c]{@{}l@{}} ---\end{tabular} & no other data & bounding box \\ \hline
VaMoS & $112 \times 112$ & ResNet-50 & \begin{tabular}[c]{@{}l@{}}Additive Angular \\ Margin \end{tabular} & only provided data & \begin{tabular}[c]{@{}l@{}}bounding box +\\ landmarks\end{tabular} \\ \hline
\end{tabular}}
\vspace{0.4mm}
\caption{Basic details of the submitted approaches. ResNet-50 is the most common utilized model architecture in the competition and the used input size varies. More details on the submitted algorithms are provided in Section  \ref{solutions}.}
\label{approaches}
\end{table*}
